ESAFL: Efficient Secure Additively Homomorphic Encryption for Cross-Silo Federated Learning

Cross-silo federated learning (FL) enables multiple clients to collaboratively train a machine learning model without sharing training data, but privacy in FL remains a major challenge. Techniques using homomorphic encryption (HE) have been designed to solve this but bring their own challenges. Many techniques using single-key HE (SKHE) require clients to fully trust each other to prevent privacy disclosure between clients. However, fully trusted clients are hard to ensure in practice. Other techniques using multi-key HE (MKHE) aim to protect privacy from untrusted clients but lead to the disclosure of training results in public channels by untrusted third parties, e.g., the public cloud server. Besides, MKHE has higher computation and communication complexity compared with SKHE. We present a new FL protocol ESAFL that leverages a novel efficient and secure additively HE (ESHE) based on the hard problem of ring learning with errors. ESAFL can ensure the security of training data between untrusted clients and protect the training results against untrusted third parties. In addition, theoretical analyses present that ESAFL outperforms current techniques using MKHE in computation and communication, and intensive experiments show that ESAFL achieves approximate 204 times-953 times and 11 times-14 times training speedup while reducing the communication burden by 77 times-109 times and 1.25 times-2 times compared with the state-of-the-art FL models using SKHE.

==> sections/0-abstract.tex <==
 \IEEEtitleabstractindextext{
 \begin{abstract}
  %
  Cross-silo federated learning (FL) enables multiple clients to collaboratively train a machine learning model without sharing training data, but privacy in FL remains a major challenge.
  Techniques using homomorphic encryption (HE) have been designed to solve this, but bring their own challenges.
  Many techniques using single-key HE (SKHE) require clients to fully trust each other to prevent privacy disclosure between clients. However, fully trusted clients are hard to ensure in practice.
  Other techniques using multi-key HE (MKHE) aims to protect privacy from untrusted clients, but lead to the disclosure of training results by untrusted third parties, e.g., the public cloud server.
  Besides, MKHE still faces the potential threat of privacy disclosure from untrusted clients, as the clients can infer privacy-sensitive information though comparing ciphertexts of different training rounds in FL.
  In terms of efficiency, MKHE has higher computation and communication complexity compared with SKHE.
  We present a new FL protocol \nameScheme that leverages a novel secure multiparty HE (MPHE) based on the hard problem of ring learning with errors.
  \nameScheme can ensure the security of training data between untrusted clients and protect the training results against
  untrusted third parties. %, and prevent privacy disclosure over multiple training rounds.
  In addition, theoretical analyses present that \nameScheme outperforms current techniques using MKHE in computation and communication, and intensive experiments show that \nameScheme achieves approximate $204\times$-$953\times$ and $11\times$-$14\times$ training speedup while reducing the communication burden by $77\times$-$109\times$ and $1.25\times$-$2\times$ compared with the state-of-the-art FL models using SKHE.

\end{abstract}

\begin{IEEEkeywords}
Federated learning, privacy protection, homomorphic encryption, secure addition computation.
\end{IEEEkeywords}}

